Application-driven Design Exploration for Dense Ferroelectric Embedded Non-volatile Memories

The memory wall bottleneck is a key challenge across many data-intensive applications. Multi-level FeFET-based embedded non-volatile memories are a promising solution for denser and more energy-efficient on-chip memory. However, reliable multi-level cell storage requires careful optimizations to minimize the design overhead costs. In this work, we investigate the interplay between FeFET device characteristics, programming schemes, and memory array architecture, and explore different design choices to optimize performance, energy, area, and accuracy metrics for critical data-intensive workloads. From our cross-stack design exploration, we find that we can store DNN weights and social network graphs at a density of over 8MB/mm^2 and sub-2ns read access latency without loss in application accuracy.

==> tables/app_results.tex <==
\begin{table}[b]
\vspace{-0.2in}
\caption{Summary of minimal cell size per programming scheme without application accuracy degradation, as discussed in Section \ref{sec:eval}.}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Workload}          & \textbf{Bits Per Cell} & \textbf{Programming} & \textbf{Minimum \# Domains} \\ \hline
\multirow{4}{*}{ResNet18}  & 1                      & Single Pulse                & 300                         \\ \cline{2-4} 
                           & 1                      & With Verify                 & 50                         \\ \cline{2-4} 
                           & 2                      & With Verify                 & 150                        \\ \cline{2-4} 
                           & 3                      & With Verify                 & 400                        \\ \hline
\multirow{4}{*}{ALBERT}    & 1                      & Single Pulse                & 200                         \\ \cline{2-4} 
                           & 1                      & With Verify                 & 50                         \\ \cline{2-4} 
                           & 2                      & With Verify                 & 150                        \\ \cline{2-4} 
                           & 3                      & With Verify                 & 150                        \\ \hline
\multirow{4}{*}{Wikipedia} & 1                      & Single Pulse                & 250                         \\ \cline{2-4} 
                           & 1                      & With Verify                 & 50                          \\ \cline{2-4} 
                           & 2                      & With Verify                 & 150                         \\ \cline{2-4} 
                           & 3                      & With Verify                 & 400                         \\ \hline
\multirow{4}{*}{Facebook}  & 1                      & Single Pulse                & 250                         \\ \cline{2-4} 
                           & 1                      & With Verify                 & 20                          \\ \cline{2-4} 
                           & 2                      & With Verify                 & 150                         \\ \cline{2-4} 
                           & 3                      & With Verify                 & 200                         \\ \hline
\end{tabular}

\label{tab:apps}
\end{table}
